LLM-Based Test-Driven Interactive Code Generation: User Study and Empirical Evaluation

Large language models (LLMs) have shown great potential in automating significant aspects of coding by producing natural code from informal natural language (NL) intent. However, given NL is informal, it does not lend easily to checking that the generated code correctly satisfies the user intent. In this paper, we propose a novel interactive workflow TiCoder for guided intent clarification (i.e., partial formalization) through tests to support the generation of more accurate code suggestions. Through a mixed methods user study with 15 programmers, we present an empirical evaluation of the effectiveness of the workflow to improve code generation accuracy. We find that participants using the proposed workflow are significantly more likely to correctly evaluate AI generated code, and report significantly less task-induced cognitive load. Furthermore, we test the potential of the workflow at scale with four different state-of-the-art LLMs on two python datasets, using an idealized proxy for a user feedback. We observe an average absolute improvement of 45.97% in the pass@1 code generation accuracy for both datasets and across all LLMs within 5 user interactions, in addition to the automatic generation of accompanying unit tests.

==> body/background.tex <==
\section{Background}
\label{sec:background}



==> body/experiments.tex <==
\section{Research Questions}




==> body/rqs/rq2.tex <==

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/t46-time.png}
    \caption{ }
    \label{fig:rq2-time}
\end{figure}


\subsection{RQ2: \rqb}
\sarah{few considerations... the results are very nuanced and may not have enough space to get the message across without raising more questions. For e.g. why is cogload opposite to time taken. The task setup also takes a lot of extra space.}
For this research question we are interested in understanding how different test validation techniques, namely asking the user to validate a test output in Assistant 2 or asking the user to provide the output as in Assistant 3, impacts developers' performance. 

We analyze the impact of each AI Assistant both across and within tasks, on the three metrics: time, correctness, and cognitive load. We use an independent t-test to compare the means for Assistants 2 and 3 for each task, and a mixed-effects model to compare effects across tasks. We report the means in Table~\ref{tab:t46}. Both the results of the independent t-test and mixed-effects models showed that there is no significant impact of the Assistant condition on any of the measured variables.  

Although the effects are not significant, we do notice trends in the differences of the means between participants using Assistants 2 and those using Assistant 3. We also observe differences among participant behavior for each task. We discuss these findings next. 

\subsubsection{For certain tasks, verifying the given output of a test case may be faster, and less cognitively demanding, than calculating the output}

For task 4, RemoveChars, we observe that participants that validate the output of test take less time, on average 30\% faster, than those asked to provide the output, with a mean of 69.16 seconds with Assistant 2 and 103.00 seconds in Assistant 3.  For this specific task, providing the output requires parsing the input string character by character, and removing each value that is specified in the second input string. However, when validating the output, the participant only has to check if the output strings contains any 'forbidden' characters from the second input string. If the output contains a forbidden character, then the participant can directly evaluate the test to be false, which provides a shortcut to mentally calculating the full return string, in the case of Assistant 3. 

We see a similar trend for task 6, Sum, where some participants are able to more quickly validate if the sum of all elements of a tuple is equal to the output value. 2 out of 4 of the AI generated tests shown in Assistant 2 contain arithmetic bugs. However, these bugs were easy to spot as they were off by 5 or 10, and not subtle errors. 

\sarah{task 5, lower mean without outliers, but much higher distribution for a2, due to double checking when incorrect}



\subsubsection{Participants may make mistakes in both test validation techniques}

\sarah{discussion on errors in each task}

\subsubsection{Regardless of validation technique, tests provide a concrete artifact from which participants can build their mental model of the problem task.}

\sarah{anec from tasks 1-3}

\sarah{add discussion prompting Benchmark}

\begin{table}[]
\begin{tabular}{@{}lllll@{}}
\toprule
Metric & Treatment & Task 4 & Task 5 & Task 6 \\ \midrule
Cognitive Load (0-100) & Assistant 2 & 22.33 & 11.00 & 19.12 \\
 & Assistant 3 & 17.87 & 15.14 & 14.71 \\ \midrule
Time (seconds) & Assistant 2 & 69.16 & 96.0 & 61.75 \\
 & Assistant 3 & 103.00 & 73.71 & 88.14 \\ \midrule
Correctness (\% tests) & Assistant 2 & 91\% & 93\% & 100\% \\
 & Assistant 3 & 96\% & 91\% & 100\% \\ \bottomrule
\end{tabular}
\label{tab:t46}
\end{table}

==> body/rqs/rq4.tex <==

\subsection{RQ4: \rqd}
\label{sec:rq4}

